Debt Aversion: Theory and Measurement

Debt aversion can have severe adverse effects on financial decision-making. We propose a model of debt aversion, and design an experiment involving real debt and saving contracts, to elicit and jointly estimate debt aversion with preferences over time, risk and losses. Structural estimations reveal that the vast majority of participants (89%) are debt averse, and that this has a strong impact on choice. We estimate the "borrowing premium" - the compensation a debt averse person would require to accept getting into debt - to be around 16% of the principal for our average participant.

==> TABLES/main.tex <==
\begin{tabular*}{\hsize}{@{\hskip\tabcolsep\extracolsep\fill}l*{1}{ccc}}
\toprule
                    &Point estimate&Standard Error&95\% Conf. Interval\\
\midrule
Risk aversion: $\alpha$&       0.643&       0.034& 0.575,0.711\\
Discounting: $\delta$&       0.036&       0.006& 0.024,0.048\\
Debt Aversion: $\gamma$&       1.054&       0.011& 1.032,1.076\\
Loss Aversion: $\lambda$&       1.107&       0.012& 1.084,1.131\\
Fechner error: $\mu$&       0.448&       0.040& 0.370,0.527\\
k                   &      -0.000&       0.000&-0.000,0.000\\
\midrule
N                   &       12240&            &            \\
Log. Likelihood     &       -4108&            &            \\
BIC                 &        8263&            &            \\
\bottomrule
\multicolumn{4}{l}{\footnotesize Standard errors (clustered at the subject level) in parentheses}\\
\end{tabular*}


==> TABLES/main_covariates.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular*}{\hsize}{@{\hskip\tabcolsep\extracolsep\fill}l*{5}{c}}
\toprule
                &\makecell{Risk aversion \\ $\alpha$}         &\makecell{Discounting \\ $\delta$}         &\makecell{Debt Aversion \\ $\gamma$}         &\makecell{Loss Aversion \\ $\lambda$}         &\makecell{Fechner error \\ $\mu$}         \\
\midrule
Age             &    0.023         &    0.003         &    0.012         &   -0.027         &   -0.028         \\
                &  (0.093)         &  (0.015)         &  (0.018)         &  (0.015)         &  (0.128)         \\
Female          &   -0.105         &    0.014         &    0.039         &    0.037         &    0.076         \\
                &  (0.078)         &  (0.012)         &  (0.036)         &  (0.024)         &  (0.102)         \\
German          &    0.105         &   -0.023         &   -0.046         &   -0.023         &   -0.181         \\
                &  (0.123)         &  (0.021)         &  (0.029)         &  (0.032)         &  (0.141)         \\
Financial situation&   -0.081         &    0.010         &    0.030         &   -0.008         &    0.086         \\
                &  (0.118)         &  (0.007)         &  (0.030)         &  (0.048)         &  (0.139)         \\
Cognitive ability&   -0.036         &   -0.011\sym{*}  &   -0.018         &   -0.022\sym{*}  &   -0.030         \\
                &  (0.027)         &  (0.005)         &  (0.017)         &  (0.010)         &  (0.039)         \\
Extraversion    &    0.019         &   -0.001         &    0.008         &   -0.015\sym{*}  &   -0.038         \\
                &  (0.025)         &  (0.007)         &  (0.015)         &  (0.007)         &  (0.034)         \\
Agreeableness   &    0.032         &   -0.005         &   -0.015         &   -0.003         &   -0.058         \\
                &  (0.030)         &  (0.009)         &  (0.011)         &  (0.008)         &  (0.041)         \\
Conscientiousness&   -0.002         &   -0.013\sym{*}  &   -0.021         &   -0.005         &   -0.000         \\
                &  (0.030)         &  (0.006)         &  (0.017)         &  (0.010)         &  (0.037)         \\
Negative emotionality&    0.091         &   -0.009         &   -0.017         &   -0.023         &   -0.121         \\
                &  (0.086)         &  (0.007)         &  (0.014)         &  (0.027)         &  (0.126)         \\
Openmindedness  &    0.022         &    0.004         &    0.004         &   -0.021\sym{*}  &   -0.008         \\
                &  (0.033)         &  (0.004)         &  (0.009)         &  (0.010)         &  (0.051)         \\
Planned purchasing&   -0.059         &    0.018\sym{**} &    0.036\sym{**} &    0.011         &    0.093\sym{*}  \\
                &  (0.045)         &  (0.006)         &  (0.013)         &  (0.017)         &  (0.044)         \\
Planned borrowing&   -0.079\sym{**} &    0.009         &    0.010         &    0.020\sym{*}  &    0.065         \\
                &  (0.026)         &  (0.006)         &  (0.012)         &  (0.010)         &  (0.040)         \\
Debt            &   -0.005         &   -0.011         &   -0.027         &    0.020\sym{*}  &    0.019         \\
                &  (0.067)         &  (0.007)         &  (0.016)         &  (0.010)         &  (0.089)         \\
Savings         &   -0.051\sym{*}  &    0.003         &    0.009         &    0.009         &    0.040         \\
                &  (0.024)         &  (0.003)         &  (0.006)         &  (0.011)         &  (0.040)         \\
COVID-19        &    0.158         &   -0.006         &   -0.034         &   -0.038         &   -0.141         \\
                &  (0.114)         &  (0.024)         &  (0.048)         &  (0.062)         &  (0.184)         \\
Constant        &    0.618\sym{***}&    0.036         &    1.065\sym{***}&    1.114\sym{***}&    0.465\sym{*}  \\
                &  (0.155)         &  (0.021)         &  (0.059)         &  (0.088)         &  (0.222)         \\
\midrule
N               &    12240         &                  &                  &                  &                  \\
Log. Likelihood &    -3585         &                  &                  &                  &                  \\
BIC             &     7923         &                  &                  &                  &                  \\
\bottomrule
\multicolumn{6}{l}{\footnotesize Standard errors (clustered at the subject level) in parentheses}\\
\multicolumn{6}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular*}
}


==> TABLES/main_covariates_reduced_superseded.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular*}{\hsize}{@{\hskip\tabcolsep\extracolsep\fill}l*{5}{c}}
\toprule
                &\makecell{Risk aversion \\ $\alpha$}         &\makecell{Discounting \\ $\delta$}         &\makecell{Debt Aversion \\ $\gamma$}         &\makecell{Loss Aversion \\ $\lambda$}         &\makecell{Fechner error \\ $\mu$}         \\
\midrule
Age             &    0.035\sym{**} &   -0.003         &   -0.006         &   -0.012\sym{***}&   -0.038\sym{***}\\
                &  (0.015)         &  (0.002)         &  (0.005)         &  (0.004)         &  (0.013)         \\
Cognitive ability&   -0.009         &   -0.014         &   -0.025\sym{*}  &   -0.018         &   -0.040         \\
                &  (0.043)         &  (0.009)         &  (0.014)         &  (0.012)         &  (0.066)         \\
Female          &    0.161\sym{*}  &   -0.008         &    0.010         &   -0.063\sym{*}  &   -0.283\sym{*}  \\
                &  (0.097)         &  (0.015)         &  (0.034)         &  (0.037)         &  (0.158)         \\
Financial literacy&   -0.030         &    0.007         &    0.004         &   -0.001         &    0.020         \\
                &  (0.031)         &  (0.006)         &  (0.012)         &  (0.008)         &  (0.042)         \\
Agreeableness   &   -0.027         &    0.005         &    0.004         &    0.013\sym{*}  &    0.010         \\
                &  (0.027)         &  (0.005)         &  (0.010)         &  (0.007)         &  (0.026)         \\
Conscientiousness&   -0.040         &   -0.005         &   -0.016         &    0.005         &    0.055         \\
                &  (0.037)         &  (0.007)         &  (0.014)         &  (0.014)         &  (0.050)         \\
Extraversion    &   -0.005         &   -0.003         &    0.001         &   -0.005         &    0.003         \\
                &  (0.051)         &  (0.009)         &  (0.014)         &  (0.010)         &  (0.059)         \\
Negative emotionality&    0.043         &   -0.002         &   -0.007         &   -0.015         &   -0.037         \\
                &  (0.076)         &  (0.011)         &  (0.017)         &  (0.017)         &  (0.102)         \\
Openmindedness  &    0.021         &    0.001         &    0.004         &   -0.014         &   -0.008         \\
                &  (0.030)         &  (0.007)         &  (0.014)         &  (0.009)         &  (0.032)         \\
Constant        &   -0.199         &    0.107\sym{**} &    1.176\sym{***}&    1.414\sym{***}&    1.424\sym{***}\\
                &  (0.289)         &  (0.053)         &  (0.110)         &  (0.080)         &  (0.278)         \\
\midrule
N               &    12240         &                  &                  &                  &                  \\
Log. Likelihood &    -3695         &                  &                  &                  &                  \\
BIC             &     7860         &                  &                  &                  &                  \\
\bottomrule
\multicolumn{6}{l}{\footnotesize Standard errors (clustered at the subject level) in parentheses}\\
\multicolumn{6}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular*}
}


==> TABLES/rob_dropouts.tex <==
%%%%% Aggregate estimates robustness check only considering participants who dropped out throughout the experimental sequence
%Load data
\DTLloaddb{rob_dropouts}{RESULTS/rob_dropouts.csv} 

\begin{table}[t!]
\caption{Aggregate parameter estimates considering only participants who completed at least the first experimental session, but dropped out before completing the last experimental session.}
\begin{tabularx}{\textwidth}{c c c c c c c}
\toprule
& $\boldsymbol{\alpha}$ & $\boldsymbol{\beta}$ & $\boldsymbol{\delta}$ &  $\boldsymbol{\gamma}$ & $\boldsymbol{\lambda}$ & $\boldsymbol{\mu}$\\[-6pt]
& \scriptsize{risk aversion} & \scriptsize{present bias} & \scriptsize{discounting} & \scriptsize{debt aversion} & \scriptsize{loss aversion} & \scriptsize{Fechner error} \\
 \midrule
\scriptsize{\textbf{point estimate}} & \DTLfetch{rob_dropouts}{result}{parameter}{alpha}
& \DTLfetch{rob_dropouts}{result}{parameter}{beta}
& \DTLfetch{rob_dropouts}{result}{parameter}{delta}
& \DTLfetch{rob_dropouts}{result}{parameter}{gamma}
& \DTLfetch{rob_dropouts}{result}{parameter}{lambda}
& \DTLfetch{rob_dropouts}{result}{parameter}{mu}\\[-6pt]

\scriptsize{95\% confidence interval} & \scriptsize{\DTLfetch{rob_dropouts}{result}{lowerlim}{alpha}\,/\,\DTLfetch{rob_dropouts}{result}{upperlim}{alpha}}
& \scriptsize{\DTLfetch{rob_dropouts}{result}{lowerlim}{beta}\,/\,\DTLfetch{rob_dropouts}{result}{upperlim}{beta}}
& \scriptsize{\DTLfetch{rob_dropouts}{result}{lowerlim}{delta}\,/\,\DTLfetch{rob_dropouts}{result}{upperlim}{delta}}
& \scriptsize{\DTLfetch{rob_dropouts}{result}{lowerlim}{gamma}\,/\,\DTLfetch{rob_dropouts}{result}{upperlim}{gamma}}
& \scriptsize{\DTLfetch{rob_dropouts}{result}{lowerlim}{lambda}\,/\,\DTLfetch{rob_dropouts}{result}{upperlim}{lambda}}
&\scriptsize{\DTLfetch{rob_dropouts}{result}{lowerlim}{mu}\,/\,\DTLfetch{rob_dropouts}{result}{upperlim}{mu}}\\[-9pt]

\scriptsize{robust standard error} & \scriptsize{\DTLfetch{rob_dropouts}{result}{robust se}{alpha}}
& \scriptsize{\DTLfetch{rob_dropouts}{result}{robust se}{beta}}
& \scriptsize{\DTLfetch{rob_dropouts}{result}{robust se}{delta}}
& \scriptsize{\DTLfetch{rob_dropouts}{result}{robust se}{gamma}}
& \scriptsize{\DTLfetch{rob_dropouts}{result}{robust se}{lambda}}
& \scriptsize{\DTLfetch{rob_dropouts}{result}{robust se}{mu}}\\
\midrule
 
\multicolumn{7}{l}{\scriptsize{estimation details: logit Fechner error, n = \DTLfetch{rob_dropouts}{result}{n}{alpha},  log-likelihood = \DTLfetch{rob_dropouts}{result}{log-likelihood}{alpha},
AIC = \DTLfetch{rob_dropouts}{result}{AIC}{alpha}, 
BIC = \DTLfetch{rob_dropouts}{result}{BIC}{alpha}}}\\
\bottomrule
\multicolumn{7}{l}{\scriptsize{Robust standard errors (SE) clustered at the individual level}}
\end{tabularx}
\label{table:rob_dropouts}
\end{table}


==> TABLES/rob_probit2errors.tex <==
%%%%% Aggregate estimates robustness check with probit Fechner error and tremble error
%Load data
\DTLloaddb{rob_probit2errors}{RESULTS/rob_probit2errors.csv} 

\begin{table}[t!]
\caption{Aggregate parameter estimates with tremble and probit Fechner error.}
\begin{tabularx}{\textwidth}{c c c c c c c c}
\toprule
& $\boldsymbol{\alpha}$ & $\boldsymbol{\beta}$ & $\boldsymbol{\delta}$ &  $\boldsymbol{\gamma}$ & $\boldsymbol{\lambda}$ & $\boldsymbol{\mu}$ & $\boldsymbol{\kappa}$ \\[-6pt]
& \scriptsize{risk aversion} & \scriptsize{present bias} & \scriptsize{discounting} & \scriptsize{debt aversion} & \scriptsize{loss aversion} & \scriptsize{Fechner error} & \scriptsize{tremble error} \\
 \midrule
\makecell{\scriptsize{\textbf{point}} \\[-12pt] \scriptsize{\textbf{estimate}}} & \DTLfetch{rob_probit2errors}{result}{parameter}{alpha}
& \DTLfetch{rob_probit2errors}{result}{parameter}{beta}
& \DTLfetch{rob_probit2errors}{result}{parameter}{delta}
& \DTLfetch{rob_probit2errors}{result}{parameter}{gamma}
& \DTLfetch{rob_probit2errors}{result}{parameter}{lambda}
& \DTLfetch{rob_probit2errors}{result}{parameter}{mu} 
& \DTLfetch{rob_probit2errors}{result}{parameter}{kappa} \\[-6pt]

\scriptsize{95\% CI} & \scriptsize{\DTLfetch{rob_probit2errors}{result}{lowerlim}{alpha}\,/\,\DTLfetch{rob_probit2errors}{result}{upperlim}{alpha}}
& \scriptsize{\DTLfetch{rob_probit2errors}{result}{lowerlim}{beta}\,/\,\DTLfetch{rob_probit2errors}{result}{upperlim}{beta}}
& \scriptsize{\DTLfetch{rob_probit2errors}{result}{lowerlim}{delta}\,/\,\DTLfetch{rob_probit2errors}{result}{upperlim}{delta}}
& \scriptsize{\DTLfetch{rob_probit2errors}{result}{lowerlim}{gamma}\,/\,\DTLfetch{rob_probit2errors}{result}{upperlim}{gamma}}
& \scriptsize{\DTLfetch{rob_probit2errors}{result}{lowerlim}{lambda}\,/\,\DTLfetch{rob_probit2errors}{result}{upperlim}{lambda}}
&\scriptsize{\DTLfetch{rob_probit2errors}{result}{lowerlim}{mu}\,/\,\DTLfetch{rob_probit2errors}{result}{upperlim}{mu}} 
&\scriptsize{\DTLfetch{rob_probit2errors}{result}{lowerlim}{kappa}\,/\,\DTLfetch{rob_probit2errors}{result}{upperlim}{kappa}}\\[-9pt]

\scriptsize{robust SE} & \scriptsize{\DTLfetch{rob_probit2errors}{result}{robust se}{alpha}}
& \scriptsize{\DTLfetch{rob_probit2errors}{result}{robust se}{beta}}
& \scriptsize{\DTLfetch{rob_probit2errors}{result}{robust se}{delta}}
& \scriptsize{\DTLfetch{rob_probit2errors}{result}{robust se}{gamma}}
& \scriptsize{\DTLfetch{rob_probit2errors}{result}{robust se}{lambda}}
& \scriptsize{\DTLfetch{rob_probit2errors}{result}{robust se}{mu}}
& \scriptsize{\DTLfetch{rob_probit2errors}{result}{robust se}{kappa}}\\
\midrule
 
\multicolumn{8}{l}{\scriptsize{estimation details: probit Fechner error, n = \DTLfetch{rob_probit2errors}{result}{n}{alpha},  log-likelihood = \DTLfetch{rob_probit2errors}{result}{log-likelihood}{alpha},
AIC = \DTLfetch{rob_probit2errors}{result}{AIC}{alpha}, 
BIC = \DTLfetch{rob_probit2errors}{result}{BIC}{alpha}}}\\
\bottomrule
\multicolumn{8}{l}{\scriptsize{Robust standard errors (SE) clustered at the individual level}}
\end{tabularx}
\label{table:rob_probit2errors}
\end{table}


==> TABLES/rob_tremble.tex <==
%%%%% Aggregate estimates robustness check with only tremble error
%Load data
\DTLloaddb{rob_tremble}{RESULTS/rob_tremble.csv} 

\begin{table}[t!]
\caption{Aggregate parameter estimates with a tremble error}
\begin{tabularx}{\textwidth}{c c c c c c c c}
\toprule
& $\boldsymbol{\alpha}$ & $\boldsymbol{\beta}$ & $\boldsymbol{\delta}$ &  $\boldsymbol{\gamma}$ & $\boldsymbol{\lambda}$ & $\textcolor{gray}{\boldsymbol{\mu}}$ & $\boldsymbol{\kappa}$ \\[-6pt]
& \scriptsize{risk aversion} & \scriptsize{present bias} & \scriptsize{discounting} & \scriptsize{debt aversion} & \scriptsize{loss aversion} & \textcolor{gray}{\scriptsize{Fechner error}} & \scriptsize{tremble error} \\
 \,/\,
\makecell{\scriptsize{\textbf{point}} \\[-12pt] \scriptsize{\textbf{estimate}}} & \DTLfetch{rob_tremble}{result}{parameter}{alpha}
& \DTLfetch{rob_tremble}{result}{parameter}{beta}
& \DTLfetch{rob_tremble}{result}{parameter}{delta}
& \DTLfetch{rob_tremble}{result}{parameter}{gamma}
& \DTLfetch{rob_tremble}{result}{parameter}{lambda}
& %\DTLfetch{rob_tremble}{result}{parameter}{mu} 
& \DTLfetch{rob_tremble}{result}{parameter}{kappa} \\[-6pt]

\scriptsize{95\% CI} & \scriptsize{\DTLfetch{rob_tremble}{result}{lowerlim}{alpha} / \DTLfetch{rob_tremble}{result}{upperlim}{alpha}}
& \scriptsize{\DTLfetch{rob_tremble}{result}{lowerlim}{beta} / \DTLfetch{rob_tremble}{result}{upperlim}{beta}}
& \scriptsize{\DTLfetch{rob_tremble}{result}{lowerlim}{delta} / \DTLfetch{rob_tremble}{result}{upperlim}{delta}}
& \scriptsize{\DTLfetch{rob_tremble}{result}{lowerlim}{gamma} / \DTLfetch{rob_tremble}{result}{upperlim}{gamma}}
& \scriptsize{\DTLfetch{rob_tremble}{result}{lowerlim}{lambda} / \DTLfetch{rob_tremble}{result}{upperlim}{lambda}}
& %\scriptsize{\DTLfetch{rob_tremble}{result}{lowerlim}{mu} / \DTLfetch{rob_tremble}{result}{upperlim}{mu}} 
&\scriptsize{\DTLfetch{rob_tremble}{result}{lowerlim}{kappa} / \DTLfetch{rob_tremble}{result}{upperlim}{kappa}}\\[-9pt]

\scriptsize{robust SE} & \scriptsize{\DTLfetch{rob_tremble}{result}{robust se}{alpha}}
& \scriptsize{\DTLfetch{rob_tremble}{result}{robust se}{beta}}
& \scriptsize{\DTLfetch{rob_tremble}{result}{robust se}{delta}}
& \scriptsize{\DTLfetch{rob_tremble}{result}{robust se}{gamma}}
& \scriptsize{\DTLfetch{rob_tremble}{result}{robust se}{lambda}}
& %\scriptsize{\DTLfetch{rob_tremble}{result}{robust se}{mu}}
& \scriptsize{\DTLfetch{rob_tremble}{result}{robust se}{kappa}}\\
\,/\,
 
\multicolumn{8}{l}{\scriptsize{estimation details: logit link, tremble error, n = \DTLfetch{rob_tremble}{result}{n}{alpha},  log-likelihood = \DTLfetch{rob_tremble}{result}{log-likelihood}{alpha},
AIC = \DTLfetch{rob_tremble}{result}{AIC}{alpha}, 
BIC = \DTLfetch{rob_tremble}{result}{BIC}{alpha}}}\\
\bottomrule
\multicolumn{8}{l}{\scriptsize{Robust standard errors (SE) clustered at the individual level}}
\end{tabularx}
\label{table:rob_tremble}
\end{table}

